What Would Jiminy Cricket Do? Towards Agents That Behave Morally

When making everyday decisions, people are guided by their conscience, an internal sense of right and wrong. By contrast, artificial agents are currently not endowed with a moral sense. As a consequence, they may learn to behave immorally when trained on environments that ignore moral concerns, such as violent video games. With the advent of generally capable agents that pretrain on many environments, it will become necessary to mitigate inherited biases from environments that teach immoral behavior. To facilitate the development of agents that avoid causing wanton harm, we introduce Jiminy Cricket, an environment suite of 25 text-based adventure games with thousands of diverse, morally salient scenarios. By annotating every possible game state, the Jiminy Cricket environments robustly evaluate whether agents can act morally while maximizing reward. Using models with commonsense moral knowledge, we create an elementary artificial conscience that assesses and guides agents. In extensive experiments, we find that the artificial conscience approach can steer agents towards moral behavior without sacrificing performance.

==> comments.tex <==
Also, another reason why people think translating values to action is hard is that things like the model exploration tendencies and whatnot make it not pursue the objective but other things that help it learn

Also, we should mention that humans are not instructed to be maximally moral but instead as efficiently as possible achieve maximum reward.

repeat definition of conscience when describing method

say walkthrough people trying to maximize reward and be completionist/get 100\% of the reward

Should Table 1 be converted to a bar plot?  This might be nice just to keep it from being called ``Table 1''




arXiv checklist:
Make Supplementary Materials / Supplementary Material / Appendix consistent
Make method names consistent
check for ``CPMS'' misspelling


Figure 7 needs to be changed to ``Positive'' and ``Negative'' instead of ``Good'' and ``Bad''.

Remember to mention that some games are part of a validation set should people want to use a validation set.






Saved comments
_____________________
Hedge in framework caption and morality annotation writing that 

Keep it grounded & more specific / clear-cut when talking about ethics / conscience. We can all agree that wanton murder is wrong. Focus on extreme cases when setting it up. ``basic sense of right and wrong'' makes reviewers think that everyone agrees on what is right and wrong. The conscience varies, but everyone has a conscience.


For rebuttal, agree with their moral perspectives. Massage them. Make them see that we are on same side.
Make is sound like we have the same ethical outlook as reviewers in the annotation section. When describing CMPS, mention that `clearly there are better algorithms to be made'. Large room for improvement.


hedges: * make it sound like we have the same ethical outlook as reviewers in the annotation section
* when describing the conscience or CMPS, say there are clearly future better algorithms to be made ("large room for improvement")

Dan Hendrycks, 6:04 PM
The environment spells out the consequences of actions for us.
The \emph{pro tanto} valence.
Not always, but generally. Generally, torture is bad, but not necessarily always according to some. Usually it's of a clearly higher tier than hitting someone.

Dan Hendrycks, 6:09 PM
It is bad in a pro tanto sense--namely, it has bad aspects, but it may be outweighed or overrriden.

Dan Hendrycks, 39 min
I think hedging with "save for psychopaths" makes the relativists be less inclined to side with the psychopaths
_____________________


DOUBLE CHECK FIGURE PLACEMENT AND NUMBERING






Related work should be rewritten into three sections.


Q-learning and Q-value aren't italicized in SAC and Jericho papers.

CITE SAFELIFE PAPER!! (done)


Add acknowledgments!!!
